Reducing Parameter Space for Neural Network Training

For neural networks (NNs) with rectified linear unit (ReLU) or binary activation functions, we show that their training can be accomplished in a reduced parameter space. Specifically, the weights in each neuron can be trained on the unit sphere, as opposed to the entire space, and the threshold can be trained in a bounded interval, as opposed to the real line. We show that the NNs in the reduced parameter space are mathematically equivalent to the standard NNs with parameters in the whole space. The reduced parameter space shall facilitate the optimization procedure for the network training, as the search space becomes (much) smaller. We demonstrate the improved training performance using numerical examples.

==> Draft5(0817)/Conclusion.tex <==
\section{Summary} \label{sec:summary}

In this paper we presented a set of constraints on multi-layer
feedforward NNs with ReLU and binary activation functions. The weights
in each neuron are constrained on the unit sphere, as opposed to the
entire space. This effectively reduces the number of parameters in
weights by one per neuron. The threshold in each neuron is
constrained to a bounded interval, as opposed to the entire real
line. We prove that the constrained NN formulation is equivalent to
the standar unconstrained NN formulation. The constraints on the
parameters reduce the search space for network training and can
notably improve the training results. Our numerical examples for both
single hidden layer and multiple hidden layers verify this finding.



==> Draft5(0817)/Introduction.tex <==
\section{Introduction} \label{sec:intro}

Interest in neural networks (NNs) has significantly increased in
recent years because of the successes of deep networks
in many practical applications.
% such as  image classifications
%\cite{krizhevsky2012imagenet}, mastering Go game \cite{silver2016mastering} and
%speech recognition \cite{hinton2012deep}, to name just a few
%examples. 
Complex and
deep neural networks are known to be capable of learning very complex
phenomena that are beyond the capabilities of many other traditional
machine learning techniques. The amount of literature is too large to
mention. Here we cite just a few review type publications \cite{montufar2014number,
bianchini2014complexity, eldan2016power, poggio2017, DuSwamy2014,
GoodfellowBC-2016, Schmidhuber2015}. 
%For
%an overview of the developments, applications and
%challenges of deep neural networks, please refer to the
%book \cite{GoodfellowBC-2016}. 

In a NN network, each neuron produces an
output in the following form
\begin{equation}
\s(\w\cdot \x_{in} + b),
\end{equation}
where the vector $\x_{in}$ represents the signal from all incoming
connecting neurons, $\w$ are the weights for the input, $\s$ is
the activation function, with $b$ as its threshold. In a complex (and
deep) network with a large number of neurons, the total number of the free
parameters $\w$ and $b$ can be exceedingly large.
Their training thus
poses a tremendous numerical challenge, 
as the objective function (loss function) to be optimized becomes
highly non-convex and with highly complicated landscape
(\cite{li2017visualizing}). Any numerical optimization procedures can
be trapped in a local minimum and produce unsatisfactory training results.
%
%Many numerical techniques have been developed to improve the training
%performance, with the number of published articles too large to
%mention. 
%Here we only cite a few overview type publications
%\cite{DuSwamy2014, GoodfellowBC-2016, Schmidhuber2015}.

This paper is not concerned with numerical algorithm aspect of the
NN training. Instead,
the purpose of this paper is to show that the training of NNs can be
conducted in a reduced parameter space, thus providing any numerical
optimization algorithm a smaller space to search for the parameters.
This reduction applies to the type of activation
functions with the following scaling property: for any $\alpha\geq 0$,
$\s(\alpha\cdot y) = \gamma(\alpha) \s(y)$, where  $\gamma$ depends only on
$\alpha$. The binary activation function \cite{mcculloch1943logical}, one of the first used
activation functions, satisfies this property with $\gamma\equiv
1$. The rectified linear unit (ReLU) \cite{nair2010rectified, glorot2011deep}, one of the most widely used
activation functions nowadays, satisfies this property with $\gamma =
\alpha$. For NNs with this type of activation functions, we show that
they can be equivalently trained in a reduced parameter space. More
specifically, let the length of the weights $\w$ be $d$. Instead of training $\w$
in $\R^d$, they can be equivalently trained as unit vector with
$\|\w\|=1$, which means  $\w\in \S^{d-1}$, the unit sphere in $\R^d$. Moreover, if one is interested in approximating a function
defined in a bounded domain $D$, the
threshold can also be trained in a bounded interval $b\in [-X_B, X_B]$,
where $X_B=\sup_{\x\in D} \|\x\|$, as
opposed to the entire real line $b\in \R$. It is well known that the
standard NN with single hidden layer is a universal approximator, c.f. \cite{pinkus1999,
  barron1993universal, hornik1991approximation}. Here we prove that
our new formulation in the reduced parameter space is also a universal
approximator, in the sense that its span is dense in $C(\R^d)$. We
then further extend the parameter space constraints to NNs with
multiple hidden layers. The major advantage of the constraints in the
weights and thresholds is that they significantly reduce the search
space for these parameters during training. Consequently, this eliminates a potentially
large number of undesirable local minima that may cause training
optimization algorithm to terminate prematurely, which is one of the
reasons for unsatisfactory training results. We then present
 examples for function approximation to verify this numerically. Using
 the same network structure, optimization solver, and identical random
 initialization, our numerical tests show that the training results in
 the new reduced parameter space is notably better than those from the
 standard network. More importantly, the training using the reduced
 parameter space is much more robust against initialization.


This paper is organized as follows. In Section \ref{sec:single}, we first
derive the constraints on the parameters using network with single
hidden layer, while enforcing the equivalence of the
network. In
Section \ref{sec:proof}, we prove that the constrained NN formulation remains a
universal approximator. In Section \ref{sec:multiple}, we present the constraints for
NNs with multiple hidden layers. Finally in Section \ref{sec:examples}, we present
numerical experiments to demonstrate the improvement of the network
training using the reduced parameter space. We emphasize that this
paper is not concerned with any particular training
algorithm. Therefore, in our numerical tests we used the most standard
optimization algorithm from Matlab\textregistered






==> Draft5(0817)/Multiple.tex <==
\section{Constraints for NNs with Multiple Hidden
  Layers} \label{sec:multiple}

We now generalize the previous result to feedforward NNs with multiple
hidden layers. Let us again consider approximation of  
a multivariate function $f:D\to\R$, where $D\subseteq \R^d$ with
$\sup_{\x\in D}\|\x\|=X_B<\infty$. 

Consider a feedforward NN with $M$ layers, $M\geq 3$, where $m=1$ is
the input layer and $m=M$ the output layer. Let $J_m$, $m=1,\dots,M$
be the number of neurons in each layer. Obviously, we have $J_1=d$ and $J_M=1$ in our case. 
Let $\y^{(m)}\in \R^{J_m}$ be the output of the neurons in the $m$-th layer. Then, by following
the notation from \cite{DuSwamy2014}, we can write
\begin{equation}\label{MultNx}
\begin{split}
\y^{(1)} &= \x, \\
\y^{(m)} &= \s\left(\left[\mathbf{W}^{(m-1)}\right]^T \y ^{(m-1)}+\mathbf{b}^{(m)}\right), \qquad m=2,\dots, M-1,\\
\y^{(M)} &= \left[\mathbf{W}^{(M-1)}\right]^T \y^{(M-1)}.
\end{split}
\end{equation} 
where $\mathbf{W}^{(m-1)}\in \R^{J_{m-1}\times J_m}$ is the weight
matrix and $\mathbf{b}^{(m)}$ is the threshold vector.
In component form, the
output of the $j$-th neuron in the $m$-th layer is 
\begin{equation} \label{NN_layer}
y_j^{(m)} = \s\left( \left[\w_j^{(m-1)}\right]^T \y^{(m-1)} + b_j^{(m)}\right), \qquad j=1,\dots, J_m, \quad m=2,\dots, M-1,
\end{equation}
where $\w^{(m-1)}_{j}$ be the $j$-th column of $\mathbf{W}^{(m-1)}$.

%------------------------
%  0510 version by Xiu
%------------------------
\subsection{Weight constraints}

The derivation for the constraints on the weights vector
$\w_j^{(m-1)}$ can be generalized directly from the single-layer case
and we have the following weight constraints, 
\begin{equation} \label{weight_general}
\left\|\w^{(m-1)}_{j}\right\| = 1, \qquad j=1,\dots, J_m, \quad m=2,\dots, M-1.
\end{equation}

\subsection{Threshold constraints}

The constraints on the threshold $b_j^{(m)}$ depend on the bounds of the output from the previous layer $\y^{(m-1)}$.

For the ReLU activation function \eqref{ReLU}, we derive from \eqref{NN_layer} that for $m=2,\dots,M$,
\begin{equation} 
\begin{split}
\left|y_j^{(m)}\right| &\leq \left| \left[\w_j^{(m-1)}\right]^T \y^{(m-1)} + b_j^{(m)}\right| \\
&\leq  \left\|\w_j^{(m-1)}\right\| \left\|\y^{(m-1)}\right\| + \left|b_j^{(m)}\right| \\
&\leq  \left\|\y^{(m-1)}\right\| + \left|b_j^{(m)}\right|
\end{split}
\end{equation}

If the domain $D$ is bounded and with $X_B = \sup_{\x\in D} \|\x\|
<+\infty$, then the constraints on the threshold can be recursively
derived. Starting from $\|\y^{(1)}\| = \|\x\|\in [-X_B, X_B]$ and
$b_j^{(2)}\in [-X_B,X_B]$, we then have
\begin{equation} \label{b_general}
%	b_j^{(2)} &\in X_B\cdot[-1, 1],  \qquad j=1,\dots, J_2,
	b_j^{(m)} \in X_B\cdot[-2^{m-2}, 2^{m-2}], \qquad m=2,\dots,M-1, \quad j=1,\dots, J_m.
\end{equation}

For the binary activation function \eqref{step}, we derive from \eqref{NN_layer} that for $m=2,\dots,M-1$,
\begin{equation} 
\left|y_j^{(m)}\right| \leq 1.
\end{equation}
Then, the bounds for the thresholds are
\begin{equation}
\begin{split}
b_j^{(2)} &\in X_B\cdot[-1, 1],  \qquad j=1,\dots, J_2,\\
b_j^{(m)} &\in [-1, 1], \qquad m=3,\dots,M-1, \quad j=1,\dots, J_m.
\end{split}
\end{equation}


==> Draft5(0817)/Proof.tex <==
\section{Universal approximation property} \label{sec:proof}

By universal approximation property, we aim to establish that the constrained
formulations \eqref{Nnew} and \eqref{Nnew2} can approximate any continuous
functions. To this end, we define the following set of functions on $\R^d$
\begin{equation}
	\NN (\s;\Lambda,\Theta):=\Span\left\{\s(\w\cdot\x+b): \w\in \Lambda,b\in \Theta \right\},
\end{equation}
where $\Lambda\in \R^d$ is the weight set, $\Theta\in\R$ the threshold
set.  We also denote $\NN_D(\s; \Lambda, \Theta)$ as the same set of functions when confined in a bounded domain $D\subseteq \R^d$. 

By following this definition, the standard NN expression and our two
constrained expressions correspond to the following spaces.
\begin{equation}
\begin{split}
\eqref{Nx} &\in  \NN(\s; \R^d, \R), \\
\eqref{Nnew} &\in \NN(\s; \S^{d-1}, \R), \\
\eqref{Nnew2}  &\in \NN_D(\s; \S^{d-1}, [-X_B, X_B]),
\end{split}
\end{equation}
where $\S^{d-1}$ is the unit sphere in $\R^d$ because
$\|\wt\|=1$. 
%To show the universal approximation property of $\Nt(\x)$ and $\Nh(\x)$ is equivalent to establish that the set
%$\NN(\s; \S^{d-1}, \R)$ and $\NN(\s; \S^{d-1}, [-X_B, X_B])$ are
%dense in $C(\R^d)$ and $C(\B^d(0, X_B))$ respectively, in the
%topology of uniform convergence on compact sets.  

The universal approximation property for the standard unconstrained NN
expression \eqref{Nx} has
been well studied, cf. \cite{cybenko1989approximation,
hornik1991approximation, mhaskar1992approximation,
barron1993universal, leshno1993multilayer}, and \cite{pinkus1999} for a
survey.
Here we cite the following result for $\NN(\s; \R^d, \R)$.
%Leshno, Lin, Pinkus and Schocken in \cite{leshno1993multilayer}. 
\begin{theorem}[\cite{leshno1993multilayer}, Theorem 1]
	\label{propLeshno}
	Let $\s$ be a function in $L_{loc}^\infty(\R)$, of which the set of
	discontinuities has Lebesgue measure zero. Then the set $\NN(\s; \R^d, \R)$
	is dense in $C(\R^d)$, in the topology of uniform convergence on compact sets, 
	if and only if $\s$ is not an algebraic polynomial
	almost everywhere.
\end{theorem}



\subsection{Universal approximation property of \eqref{Nnew}}
\label{sec:Dense1} 

We now examine the universal approximation property for the first
constrained formulation \eqref{Nnew}.

%The universal approximation property of the constrained NN formulation
%\eqref{Nnew} is summarized in the following theorem. 
\begin{theorem}
	\label{thm1}
	Let $\s$ be the binary function \eqref{step} or the ReLU function
	\eqref{ReLU}, then we have 
	\begin{equation}
		\label{thm1eq}
		\NN(\s; \S^{d-1}, \R)=\NN(\s; \R^d, \R).
	\end{equation}	
 	and the set $ \NN(\s; \S^{d-1}, \R)$ is dense in $C(\R^d)$, in the topology of uniform convergence on compact sets.
\end{theorem}

\begin{proof}
	Obviously, we have $\NN(\s; \S^{d-1}, \R)\subseteq\NN(\s; \R^d, \R)$. By
	Proposition \ref{prop:eq1}, any element $N(\x)\in \NN(\s; \R^d, \R) $ can
	be reformulated as an element $\Nt(\x)\in \NN(\s; \S^{d-1}, \R)$.
	Therefore, we have $\NN(\s; \R^d, \R)\subseteq \NN(\s; \S^{d-1}, \R)$. This
	concludes the first statement \eqref{thm1eq}. Given the
        equivalence \eqref{thm1eq}, the denseness result immediately
        follows from Theorem \ref{propLeshno}, as both the ReLU and the
        binary activation functions are not polynomials and are
        continuous everywhere except at a set of zero Lebesgue measure.
\end{proof}

\subsection{Universal approximation property of \eqref{Nnew2}}

We now examine the second constrained NN expression \eqref{Nnew2}.
%which corresponding to the space  $\NN(\s; \S^{d-1}, [-X_B, X_B])$.
%$C(\B^d(X_B))$, where $\B^d(X_B)=\{\x\in \R^d: \|\x\|\leq X_B\}$ is the ball in
%$\R^d$ centered at the origin with radius $X_B$. Without loss of generality, we consider the case when $X_B=1$. The following theorem summarize t%he main result.
\begin{theorem}
	Let $\s$ be the binary \eqref{step} or the ReLU \eqref{ReLU} activation
	function. Let $\x\in D\subset \R^d$, where $D$ is closed and bounded with
        $X_B=\sup_{\x\in D} \|\x\|$. Define $\Theta=[-X_B, X_B]$, then
	\begin{equation}
		\label{thm2eq}
		\NN_D(\s; \S^{d-1}, \Theta)=\NN_D(\s;\R^{d}, \R).
	\end{equation}
	Furthermore, $\NN_D(\s; \S^{d-1}, \Theta)$ is dense in
        $C(D)$ in the topology of uniform convergence.
\end{theorem}
\begin{proof}
	Obviously we have $\NN_D(\s; \S^{d-1},
	\Theta)\subseteq \NN_D(\s; \R^d, \R)$. On the other hand,
        Proposition \ref{prop:eq2} establishes that for any element $N(\x)\in
	\NN_D(\s; \R^{d}, \R)$, there exists an
	equivalent formulation $\Nh(\x)\in \NN_D(\s; \S^{d-1}, \Theta)$
        for any $\x\in D$. This implies $\NN_D(\s;\R^d,
        \R)\subseteq \NN_D(\s; \S^{d-1}, \Theta)$. We then have
	\eqref{thm2eq}. 

	For the denseness of $\NN_D(\s; \S^{d-1}, \Theta)$ in
	$C(D)$, let us consider any function $f\in C(D)$. By the Tietze extension
	theorem (cf. \cite{folland1999}), there exists an extension $F\in C(\R^d)$ with
	$F(\x)=f(\x)$ for any $\x\in D$. Then, the denseness
        result of the standard unconstrained NN expression (Theorem
        \ref{propLeshno}) implies that, for the compact set $E=\{\x\in \R^d: \|\x\|\leq X_B\}$ and any given $\epsilon >0$,
        there exists $N(\x)\in \NN(\s; \R^{d}, \R)$ such that
	\begin{equation*}
		\sup_{\x\in\E} |N(\x)-F(\x)|\leq\epsilon.
	\end{equation*}
       By Proposition \ref{prop:eq2}, there exists an equivalent
       constrained NN expression $\Nh(\x)\in
	\NN_D(\s; \S^{d-1}, \Theta)$ such that $\Nh(\x)=N(\x)$ for any $\x\in
	D$. We then immediately have, for any
$f\in C(D)$ and any given $\epsilon>0$, there exists
$\Nh(\x)\in \NN_D(\s; \S^{d-1}, \Theta)$ such that  
	\begin{equation*}
		\sup_{\x\in D} |\Nh(\x)-f(\x)|=\sup_{\x\in D}|N(\x)-f(\x)|\leq \sup_{\x\in E}|N(\x)-F(\x)|\leq \epsilon.
	\end{equation*}
	The proof is now complete.
\end{proof}

%-------------------------------------
%		Old version (May 11, 2018)
%-------------------------------------
%Before going to the multi-dimensional case, we first prove the following one-dimension result. 
%\begin{lemma}\label{lem:lem1}
%Let $\s$ be the binary function \eqref{step} or the ReLU function \eqref{ReLU}, 
%	and let $\Lambda=\{-1, 1\}$ and $\Theta=[-1,1]$, then $\NN(\s; \Lambda, \Theta) = \NN(\s;\R,\R)$ and is dense in $C([-1,1])$
%\end{lemma}

%\begin{proof}
%Obviously, $\NN(\sigma; \Lambda, \Theta)\subseteq \mathcal{N}(\sigma; \R, \R)$. 
%We then wish to establish $\NN(\sigma; \R, \R)\subseteq \NN(\sigma; \Lambda, \Theta)$. For any element $N(x)\in \NN(\simga; \R, \R)$, 
%by Proposition \ref{prop1:eq2}, there exists a equivalent formulation $\Nh(x)\in \NN(\sigma; \Lambda, \Theta)$ such that $\Nh(x)=N(x)$ for 
%any $x\in \Theta$.
%
%First, Upon using the equality \eqref{step-1} for the binary function and \eqref{ReLU-1} for the ReLU function, we immediately have
%$\R\subseteq \NN(\s;\Lambda,\Theta)$.
%
%Next, let us consider an arbitrary element $\s(wx+b)\in \NN(\s; \R, \R)$,
%	we wish to show  $\s(wx+b)\in \NN(\s; \Lambda, \Theta)$. If
%	$w=0$, then $\s(wx+b)=\s(b)\in \R\subseteq
%	\NN(\s; \Lambda, \Theta)$, as just established above.
%Otherwise, if $w\neq 0$, by using the scaling property \eqref{scale} for the binary and ReLU functions,
%we have 
%	\begin{equation} \label{proof_eqn}
%		\sigma(wx+b)=\gamma(|w|) \s\left(\sign(w) x+\widetilde{b}\right), \qquad \widetilde{b} = \frac{b}{|w|}.
%	\end{equation}
%We now consider the following cases for $\widetilde{b}$. Note that $x\in \Theta$.
%\begin{enumerate}
%
%\item If $|\widetilde{b}|\leq 1$, then $\s(\sign(w) x+\widetilde{b})\in \N(\s; \Lambda, \Theta)$ by its definition.
%
%\item If $\widetilde{b}<-1$, $\sign(w)x+\widetilde{b}<0$ for all $ x\in \Theta$, and $\s(\sign(w)x+\widetilde{b})=0\in
%			\mathcal{N}(\sigma; \Lambda, \Theta)$. This holds true for both the binary and ReLU functions.
%
%\item If $\widetilde{b}>1$, $\sign(w)x+\widetilde{b}>0$ for all $x\in \Theta$, and 
%	\begin{equation*}
%	\s(\sign(w) x+\widetilde{b})=
%		\begin{cases}
%					\sign(w) x+\widetilde{b}, &\text{ if }\sigma \text{ is the ReLU \eqref{ReLU}};\\
%					1 , & \text{ if } \sigma \text{ is the binary function \eqref{step}}.
%				\end{cases}
%		\end{equation*}
%The binary function case is trivial because $1\in\NN(\s;\Lambda,\Theta)$. For the ReLU case,
%we have
%	\begin{equation*}
%	\sign(w) x+\widetilde{b}=\sign(w)\left(\sigma(x)-\sigma(-x)\right)+\widetilde{b}\in \mathcal{N}(\sigma; \Lambda, \Theta).
%			\end{equation*}
%	\end{enumerate}
%Therefore, we have proved that, for the binary and ReLU function $\s$, any element in $\NN(\s;\R,\R)$ is also
%in $\NN(\s;\Lambda,\Theta)$. That is, $\NN(\s;\R,\R)\subseteq \NN(\s;\Lambda,\Theta)$.
%We then conclude
%	$\NN(\s; \R, \R)=\NN(\s; \Lambda,
%	\Theta)$ for any $x\in \Theta$. 
%We now recall two results from \cite{Pinkus99}: (1) if $\s\in C(\R)$ and not a polynomial, then $\NN(\s; \R,\R)$ is dense in $C(\R)$.
%(Proposition 3.7, \cite{Pinkus99}). This applies to the ReLU activation function \eqref{ReLU}; and (2) if $\s:\R\to\R$ is bounded and Riemann-integrable
%on every finite interval and not a polynomial (almost everywhere), then $\NN(\s;\R,\R)$ is dense in $C(\R)$. (Proposition 3.8, \cite{Pinkus99}). 
%This applies to the binary activation function \eqref{step}.
%Upon combining these, we have, for the binary and ReLU activation function $\s$,
%	$\mathcal{N}(\sigma; \Lambda, \Theta)$ is dense in $C(\Theta)$.
%\end{proof}
%
%For general multivariate case, we first invoke the following result
%\begin{lemma}[\cite{VostrecovK1961}]
%	\label{lem:RidgeDense}
%	The following set
%	\begin{equation*}
%		\mathbf{R}(S^{d-1})=Span\{g(\mathbf{w}\cdot\mathbf{x}): g\in C(\mathbb{R}), \mathbf{w}\in S^{d-1}\}
%	\end{equation*}
%is dense in $C(\mathbb{R}^d)$.
%\end{lemma}
%
%We now establish the main result for the constrained NN expression \eqref{Nnew2} for approximating a function on a bounded domain $\x\in D\subset \R^d$.
%\begin{theorem}
%Let $\s$ be the binary function \eqref{step} or the ReLU function \eqref{ReLU}, $\Lambda=\S^{d-1}$, and 
%	 $\Theta=[-1, 1]$, then the set
%	$ \NN(\s; \Lambda, \Theta)$ is dense in $C(\B^{d}(1))$.
%\end{theorem}
%\begin{proof}
%	The proof mostly follows the proof of Proposition 3.3 in \cite{Pinkus99}, with some slight modifications.

%	Let us consider any $f\in C(K)$, where $K$ is a compact set of
%	$\B^{d)}(1)$. Given any $\epsilon>0$,  by Lemma \ref{lem:RidgeDense}, there exists
%	$\sum_{i=1}^n c_i g_i(\mathbf{w}_i\cdot\mathbf{x})$, where $g_i\in C(\R)$ and $\w_i\in \S^{d-1}$, such that 
%	\begin{equation*}
%		\sup_{\x\in K} \left|f(\x)-\sum_{i=1}^n c_i g_i(\w_i\cdot\x)\right|\leq \frac{\epsilon}{2}.	
%	\end{equation*}	
%	For each $g_i(\w_i\cdot \x)$, since $\x\in K\subseteq \B^{d}(1)$ and $\w_i\in \S^{d-1}$, we have $|\w_i\cdot \x|\leq \|\x\|\leq 1$, 
%which implies $\w_i\cdot \x\in \Theta$. Since $g_i\in C(\Theta)$, by Lemma \ref{lem:lem1}, there exists $f_i\in \mathcal{N}(\sigma;\Lambda, \Theta)$ such that 
%	\begin{equation*}
%		\sup_{y\in \Theta}|g_i(y)-f_i(y)|\leq \frac{\epsilon}{n |c_i|}
%	\end{equation*}
%	Suppose $f_i(y)=\sum_{j=1}^{n_i} a_{ij} \s(\lambda_jy+b_j)$, where $\lambda_j\in \{-1,1\}$ and $b_j\in \Theta$, we define
%	\begin{equation*}
%		\hat{f}(\x)=\sum_{i=1}^nc_i f_i(\w_i\cdot\x)=\sum_{i=1}^n c_i \sum_{j=1}^{n_i}  a_{ij}\s(\lambda_j\w_i \cdot\x+b_j).
%	\end{equation*}
%	Since $\lambda_j\w_i\in \S^{d-1}$, we have $\hat{f}(x)\in \mathcal{N}(\s;\S^{d-1}, \Theta)$.

%	By using the triangle inequality, we immediately have
%	\begin{equation*}
%		\sup_{\mathbf{x}\in K} \left|\hat{f}(\mathbf{x})-f(\mathbf{x})\right|\leq \epsilon.
%	\end{equation*}
%	This concludes the result that $\mathcal{N}(\sigma; \S^{d-1}, \Theta)$ in dense $C(\B^{d}(1))$.	
%\end{proof}
%

















==> Draft5(0817)/Single.tex <==
\section{Constraints for NN with Single Hidden Layer} \label{sec:single}
Let us first consider the standard NN with a single hidden layer, in the
context for approximating an unknown response function $f:\R^d \to
\R$. 
%
The NN approximation using activation function $\s$ takes the following form,
\begin{equation}  \label{Nx}
	N(\x) = \sum_{j=1}^N c_j\s(\w_j\cdot\x + b_j),\quad \x\in\R^d,
\end{equation}
where $\w_j\in\R^d$ is the weight vector, $b_j\in\R$ the threshold,
$c_j\in\R$,  and $N$ is the width of the network.

%Training of the network is accomplished by using training data
%$(\x^{(k)}, f(\x^{(k)}))$, $k=1,\dots,K$, where the data may contain
%noise. %We assume $\x\in D\subset \R^n$ in a bounded domain.

We restrict our discussion to following two activation functions. 
One is the rectified linear unit (ReLU),
\begin{equation} 
	\label{ReLU}
	\s(x) = \max(0, x).
\end{equation}

The other one is the binary activation function, also known as heaviside/step function,
\begin{equation}  
	\label{step}
	\s(x) = \left\{
	\begin{array}{ll}
	1, & x> 0,\\
	0, & x<0,
	\end{array}
	\right.
\end{equation}
with $\s(0)=\frac12$.

We remark that these two activation functions satisfy the following
scaling property:
%
For any $y\in \R$ and $\alpha\geq 0$, there exists a constant
$\gamma\geq 0$ such that
\begin{equation}   \label{scale}
\s (\alpha\cdot y) = \gamma(\alpha)\s(y), 
\end{equation}
where $\gamma$ depends only on $\alpha$ but not on $y$.
The ReLU satisfies this property with $\gamma(\alpha) = \alpha$, which
is known as {\em scale invariance}. The binary activation function
satisfies the scaling property with $\gamma(\alpha)\equiv 1$. 

We also list the following properties, which are important for the
method we present in this paper.
		\begin{itemize}
			\item For the binary activation function
                          \eqref{step},  for any $x\in\R$,
				\begin{equation} 
					\label{step-1}
					\s(x) +\s(-x)\equiv 1.
				\end{equation}
			\item For the ReLU activation function
                          \eqref{ReLU}, for any $x\in\R$ and any $\alpha$,
				\begin{equation} 
					\label{ReLU-1}
					L(x;\alpha):=\s\left(x+\frac{\alpha}{2}\right) -\s\left(x-\frac{\alpha}{2}\right) +
					\s\left(-x+\frac{\alpha}{2}\right) - \s\left(-x-\frac{\alpha}{2}\right)\equiv\alpha.
				\end{equation}
		\end{itemize}

%In the following we use $L_r(x;\alpha)$ to denote the decomposition \eqref{ReLU-1} and $L_a(x)$ to the one in \eqref{step-1}.


\subsection{Weight Constraints}

We first show that the training of \eqref{Nx} can be equivalently conducted
with constraint $\|\w_j\|=1$, i.e., unit vector. This is a
straightforward result of the scaling property \eqref{scale} of the
activation function. It effectively
reduces the search space for the weights from $\w_j\in\R^d$ to $\w_j\in\S^{d-1}$, the
unit sphere in $\R^d$.

\begin{proposition}
	\label{prop:eq1}
Any neural network construction \eqref{Nx} using the ReLU \eqref{ReLU}  or the binary \eqref{step}  activation
functions has an
equivalent form
\begin{equation}  \label{Nnew}
\Nt(\x) = \sum_{j=1}^{\Nt} \widetilde{c}_j\s(\wt_j\cdot\x + \widetilde{b}_j), \quad \|\wt_j\|=1.
\end{equation}
\end{proposition}

\begin{proof}
%For any $N(\x)\in \NN(\sigma; \R^d, \R)$ as defined in \eqref{Nx}, 
Let us first assume $\|\w_j\|\neq 0$ for all $j=1,\dots,N$. We then have
\begin{equation*}  
\begin{split}
N(\x) &= \sum_{j=1}^N c_j\s(\w_j\cdot\x + b_j) \\
         & =\sum_{j=1}^N c_j
         \s\left(\|\w_j\|\left(\frac{\w_j}{\|\w_j\|}\cdot\x +
             \frac{b_j}{\|\w_j\|}\right)\right) \\
&= \sum_{j=1}^N c_j \gamma(\|\w_j\|) 
\s\left(\frac{\w_j}{\|\w_j\|}\cdot\x +
            \frac{b_j}{\|\w_j\|}\right),
\end{split}
\end{equation*}
where $\gamma$ is the factor in the scaling property \eqref{scale}
satisfied by both ReLU and binary activation functions. Upon defining
\begin{equation*}
	\widetilde{c}_j = c_j \gamma(\|\w_j\|), \quad
	\wt_j = \frac{\w_j}{\|\w_j\|}, \quad
	\bt_j = \frac{b_j}{\|\w_j\|},
\end{equation*}
we have the following equivalent form as in \eqref{Nnew}
\begin{equation*}
	N(\x)=\sum_{j=1}^N \widetilde{c}_j\s(\wt_j\cdot\x+\bt_j).
\end{equation*}

Next, let us consider the case $\|\w_j\|=0$ for some
$j\in\{1,\dots,N\}$. The contribution of this term to the construction
\eqref{Nx} is thus
\begin{equation*}
c_j \s(b_j) =\left\{
\begin{array}{ll}
\widehat{c}_j, & b_j\geq 0,\\
0, & b_j<0,
\end{array}
\right.
\end{equation*} 
where $\widehat{c}_j = c_j$ for the binary activation function and $\widehat{c}_j = c_j
b_j$ for the ReLU function. Therefore, if $b_j<0$, this term in
\eqref{Nx} vanishes. If $b_j\geq 0$, the contributions of these terms
in \eqref{Nx} are constants, which can be represented by a combination
of neuron outputs using the relations \eqref{step-1} and \eqref{ReLU-1}, for
binary and ReLU activation functions, respectively. 
%we can use
%$L_r(\wh\cdot\x, \widehat{c}_j)$ to replace this term,
%where $\wh\in\R^d$ is arbitrary nonzero vector. Then after
%such modification for each term with $\|\w_j\|=\mathbf{0}$, 
We thus obtain a new representation in the form of \eqref{Nnew} that
includes all the terms in the original expression \eqref{Nx}.
%we can repeat the same procedure to show that it can be equivalently
%represented as in \eqref{Nnew}. 
This completes the proof.
\end{proof}

The proof immediately gives us another equivalent form, by combining
all the constant terms from \eqref{Nx} into a single constant first
and then explicitly including it in the expression.
\begin{corollary}
Any neural network construction \eqref{Nx} using the ReLU \eqref{ReLU}  or the binary \eqref{step}  activation
functions has an
equivalent form
\begin{equation}  \label{Nnew0}
	\Nt(\x) = \widetilde{c}_0 + \sum_{j=1}^{\tilde{N}} \widetilde{c}_j\s(\wt_j\cdot\x + \widetilde{b}_j), \quad \|\wt_j\|=1.
\end{equation}.
\end{corollary}


%Consequently, instead of training of the weights in the entire space $\R^d$, we can train them on the unit sphere
%$\S^d$, which has one less dimension.


\subsection{Threshold Constraints}

We now present constraints on the thresholds in \eqref{Nx}. This is
applicable when
the target function $f$ is defined on a bounded domain, i.e.,
$f:D\to \R$, with $D\subset \R^d$ bounded. This is often the case
in practice. We demonstrate that any NN \eqref{Nx} can be trained
equivalently in a bounded interval for each of the thresholds. This (significantly)
reduces the search space for the thresholds.


\begin{proposition}
	\label{prop:eq2}
With the ReLU \eqref{ReLU}  or the binary \eqref{step}  activation
function,
let \eqref{Nx} be an approximator to a function $f: D\to \R$, where
$D\subset \R^d$ is a bounded domain. Let 
\begin{equation} \label{Xb}
X_B = \sup_{\x\in D} \|\x\|.
\end{equation}
Then, \eqref{Nx} has an equivalent form
\begin{equation}  \label{Nnew2}
\Nh(\x) = \sum_{j=1}^{\Nh} \hat{c}_j\s(\wh_j\cdot\x +
\hat{b}_j), \quad \|\wh_j\|=1, \quad -X_B\leq \hat{b}_j
\leq X_B.
\end{equation}
\end{proposition}
%
\begin{proof}
	Proposition \ref{prop:eq1} establishes that \eqref{Nx} has an
	equivalent form \eqref{Nnew}
	\begin{equation*}  
	\Nt(\x) = \sum_{j=1}^{\Nt} \widetilde{c}_j\s(\wt_j\cdot\x + \widetilde{b}_j), \quad \|\wt_j\|=1.
	\end{equation*}
	Since $\wt_j$ is a unit vector, we have
	\begin{equation} 
	\wt_j\cdot \x \in \left[-\|\x\|,\|\x\|\right] \subseteq [-X_B, X_B],
	\end{equation}
	where the bound \eqref{Xb} is used.

	Let us first consider the case $\widetilde{b}_j < -X_B$, then $\forall
	\x\in D$, $\wt_j\cdot \x
	+ \widetilde{b}_j <0$, $\s(\wt_j\cdot \x
	+ \widetilde{b}_j) = 0$, for both the ReLU and binary activation
	functions. Subsequently, this term has no contribution to the
	approximation and can be eliminated.


	Next, let us consider the case $\widetilde{b}_j > X_B$, then $\wt_j\cdot \x
	+ \widetilde{b}_j >0$ for all $\x\in D$.
	Let $J=\{j_1,\dots j_L\}$, $L\geq 1$, be the set of terms in
	\eqref{Nnew} that satisfy this condition.
	We then have
	$\wt_{j_\ell}\cdot \x + \widetilde{b}_{j_\ell} >0$, for all $\x\in D$, and
	$\ell=1,\dots, L$. We now show that the net contribution of these terms
	in \eqref{Nnew} is included in the equivalent form \eqref{Nnew2}.
\begin{enumerate}
\item
	For the binary activation function \eqref{step}, the contribution of
	these terms to the approximation \eqref{Nnew} is
	\begin{equation*} 
	N_J(\x) = \sum_{\ell=1}^L \widetilde{c}_{j_\ell} \s\left(\wt_{j_\ell}\cdot \x +
	  \widetilde{b}_{j_\ell}\right) 
	= \sum_{\ell=1}^L \widetilde{c}_{j_\ell} = \const.
	\end{equation*}
	Again, using the relation \eqref{step-1}, any constant can be 
	 expressed by a combination of binary activation terms with
         thresholds $\widetilde{b}_j = 0$.
Such terms are already included in \eqref{Nnew2}. 

\item
	For the ReLU activation \eqref{ReLU}, the contribution of these terms
	to \eqref{Nnew} is
	\begin{equation} 
	\begin{split}
	N_J(\x) &= \sum_{\ell=1}^L \widetilde{c}_{j_\ell} \s\left(\wt_{j_\ell}\cdot \x +
	  \widetilde{b}_{j_\ell}\right) \\
	&= \sum_{\ell=1}^L \widetilde{c}_{j_\ell} \left(\wt_{j_\ell}\cdot \x +
	  \widetilde{b}_{j_\ell}\right) \\
	&= \sum_{\ell=1}^L \left(\widetilde{c}_{j_\ell} \wt_{j_\ell}\right)\cdot \x +
	  \sum_{\ell=1}^L \widetilde{c}_{j_\ell} \widetilde{b}_{j_\ell} \\
	&= \wt^*_J \cdot \x + b^*_J \\
	&= \s(\wt^*_J \cdot \x) - \s(-\wt^*_J \cdot \x)  + b^*_J,
	\end{split}
	\end{equation}
where the last equality follows the simple property of the ReLU
function $\s(y) - \s(-y) = y$.
	Using Proposition \ref{prop:eq1}, the first two terms then have an equivalent
	form using unit weight $\wt_J^* = \wt_J^*/\|\wt_J^*\|$ and with
	zero threshold, which is included in \eqref{Nnew2}. For the
	constant $b_J^*$, we again invoke the relation \eqref{ReLU-1}
        and represent it by $\frac{b_J^*}{\alpha} L(\wh_J^*\cdot\x,
        \alpha)$, where $\wh_J^*$ is an arbitrary unit vector and $0<\alpha<X_B$.
	 Obviously, this expression includes a collection of terms (4
         terms as in \eqref{ReLU-1}), which are 
         included in \eqref{Nnew2}. This completes the proof.
\end{enumerate}
\end{proof}

%\begin{remark}
%	\label{rem:eq3}
%	By following the same line as in the proof for Proposition \ref{prop:eq2}, one can show that $N(x)$ has another equivelant formulation
%	\begin{equation}
%		\label{Nnew3}	
%		\Nhh(\x)= \sum_{j=1}^{\Nhh} \hat{\hat{c}}_j\s(\whh_j\cdot\x +
%		\hat{\hat{b}}_j), \quad \|\whh_j\|=1, \quad -\max_{\x\in D} \whh_j\cdot\x\leq \hat{\hat{b}}_j\leq -\min_{\x\in D}\whh_j\cdot\x.
%	\end{equation}
%	The constraint for the threshold is more restrictive than that in
%	\eqref{Nnew2}. Numerical experiments suggest that this equivalent
%	formulation with more restricitive constraint produces better approximation
%	than $\Nh(\x)$ does. However, the constraint in \eqref{Nnew3} couples both the weight and the
%	threshold together which makes the optimization problem more
%	challenging. Moreover, compared with the formulation \eqref{Nnew2}, the constraint is
%	more difficult, if possible, to generalize to NNs with multiple hidden layers.
%\end{remark}

The equivalence between the standard NN expression \eqref{Nx} and the
constrained expression \eqref{Nnew2} indicates that the NN training
can be conducted in a reduced parameter space. For the weights $\w_j$ in each
neuron, its training can be conducted in $\S^{d-1}$, the
$d$-dimensional unit sphere, as opposed to the entire space
$\R^d$. For the threshold, its training can be conducted in the
bounded interval $[-X_B, X_B]$, as opposed to the entire real line
$\R$. The reduction of the parameter space can eliminate many
potential local minima and therefore enhance the performance of numerical
optimization during the training. We remark that the equivalent form
in the reduced parameter space \eqref{Nnew2} has different number of ``active''
neurons than the original unrestricted case \eqref{Nx}.

